NOVA: Normal-Side Modeling for Training-Free Zero-Shot Video Anomaly Detection

Training-free zero-shot video anomaly detection (ZS-VAD) leverages vision-language models (VLMs) to localize anomaly instances from a predefined anomaly vocabulary, without providing any video. Existing CLIP-based methods often emphasize anomaly-side semantics, while the competing normality side remains less carefully formulated. We identify two key limitations in existing solutions: (i) blurred decision boundary: normal prompts may contain ambiguous verbs, such as running, that are semantically close to anomalies, reducing normal and abnormal separation in the VLM embedding space; and (ii) modality gap: poor alignment between features of textual normal anchors and visual frames. We propose NOVA, a training-free ZS-VAD framework that strengthens the normal side at both linguistic and visual levels. NOVA introduces Normality-Aware Prompt Construction (NA), which excludes anomaly-adjacent verbs and biases normal descriptions toward static, low-motion scenes. To overcome the text-vision modality gap, NOVA constructs a Visual Normality Anchor (VNA), which creates a weighted visual normal anchor from the initial frames of each test video, providing a video-specific normal reference without task-specific training or annotations. NOVA achieves 89.86 percent AUC on UCF-Crime and 95.07 percent AUC and 84.82 percent AP on XD-Violence, reaching state-of-the-art performance among comparable training-free zero-shot methods.

==> backup/preamble.tex <==
%% This file contains a number of tweaks that are typically applied to the main document.
%% They are not enabled by default, but can be enabled by uncommenting the relevant lines.

%%
%% Inline annotations; for predefined colors, refer to "dvipsnames" in the xcolor package:
%% https://tinyurl.com/overleaf-colors
%%
\newcommand{\red}[1]{{\color{red}#1}}
\newcommand{\blue}[1]{{\color{blue}#1}}
\newcommand{\todo}[1]{{\color{red}#1}}
\newcommand{\TODO}[1]{\textbf{\color{red}[TODO: #1]}}
%%
%% disable for camera ready / submission by uncommenting these lines  
%%
% \renewcommand{\TODO}[1]{}
% \renewcommand{\todo}[1]{#1}

%%
%% work harder in optimizing text layout. Typically shrinks text by 1/6 of page, enable
%% it at the very end of the writing process, when you are just above the page limit
%%
% \usepackage{microtype}

%%
%% fine-tune paragraph spacing
%%
% \renewcommand{\paragraph}[1]{\vspace{.5em}\noindent\textbf{#1.}}

%%
%% globally adjusts space between figure and caption
%%
% \setlength{\abovecaptionskip}{.5em}


%%
%% Allows "the use of \paper to refer to the project name"
%% with automatic management of space at the end of the word
%%
% \usepackage{xspace}
% \newcommand{\paper}{ProjectName\xspace}

%%
%% Commonly used math definitions
%%
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{arg\,max}

%%
%% Tigthen underline
%%
% \usepackage{soul}
% \setuldepth{foobar}

==> backup/sec/0_abstract.tex <==
% !TEX root = ../main.tex
\begin{abstract}
Training-free zero-shot video anomaly detection (ZS-VAD) leverages vision-language models (VLMs) to localize anomaly instances from a predefined anomaly vocabulary, without providing any training videos.
Existing CLIP-based methods often emphasize \textbf{anomaly-side semantics}, while the competing \textbf{normality side} remains less carefully formulated. We identify two key limitations in existing solutions: (i) \textbf{blurry decision boundary}: normal prompts may contain ambiguous verbs, such as ``running'', that are semantically close to anomalies, reducing normal and abnormal separation in the VLM embedding space; and (ii) \textbf{modality gap}: poor alignment between features of textual normal anchors and visual frames.

We propose \textbf{NOVA}, a training-free ZS-VAD framework that strengthens the normal side at both linguistic and visual levels. NOVA introduces \textbf{Normality-Aware Prompt Construction (NA)}, which excludes anomaly-adjacent verbs and biases normal descriptions toward static, low-motion scenes. To overcome the text-vision modality gap, NOVA constructs a \textbf{Visual Normality Anchor (VNA)} from early-frame visual embeddings of each test video, providing a per-video normal reference without requiring extra annotations or calibration. 


NOVA achieves 89.86\% AUC on UCF-Crime and 95.07\% AUC and 84.82\% AP on XD-Violence, reaching state-of-the-art performance among comparable training-free zero-shot methods.
\end{abstract}


==> backup/sec/1_intro.tex <==
% !TEX root = ../main.tex
\section{Introduction}
\label{sec:intro}

\textbf{Video Anomaly Detection (VAD)} is essential in intelligent surveillance, aiming to localize rare and semantically diverse abnormal events, such as fighting, robbery, arson, and explosions, from long and untrimmed surveillance videos. Supervised and weakly supervised methods~\cite{sultani2018real,tian2021weakly,cliptsa2022,wu2024vadclip} have achieved substantial progress in closed-set settings, but they rely on collecting and annotating anomalous samples from the target domain. This requirement is inherently restrictive: anomalies are rare, open-ended, and difficult to enumerate, making such methods less reliable when deployed in new scenes.

Vision-language models (VLMs), especially CLIP~\cite{radford2021learning}, offer a natural basis for \textbf{zero-shot VAD (ZS-VAD)} by aligning visual frames and textual event descriptions in a shared embedding space. By comparing frame-level visual embeddings against competing abnormal and normal text prompts, ZS-VAD can score anomalies that were never used for task-specific training, and 
recent methods mainly improve anomaly descriptions through richer prompts~\cite{dong2024clip,lee2025flashback}.
%recent CLIP-based methods further enrich these category-wise descriptions with LLMs~\cite{dong2024clip,lee2025flashback}.


Despite these advances, existing CLIP-based ZS-VAD methods primarily improve anomaly detection by enriching \textbf{anomaly-side semantics}. However, anomalies are inherently open-ended and difficult to describe exhaustively, making anomaly-side expansion alone insufficient. More importantly, prompt-contrastive ZS-VAD determines anomaly scores through the \textbf{relative competition} between anomaly and normal prompts rather than anomaly prompts alone. Consequently, the quality of the \textbf{normal side} directly shapes the decision boundary.
Nevertheless, normality remains underexplored in existing training-free ZS-VAD methods. Normal prompts are often treated as generic counterparts to anomaly prompts, despite normal scenes typically exhibiting stronger scene consistency and being more constrained by scene layout, object configuration, and video-specific appearance. We therefore argue that strengthening the normal side, rather than further enriching anomaly descriptions, provides a more effective direction for improving training-free ZS-VAD.

Despite these advances, existing CLIP-based ZS-VAD methods often emphasize anomaly-side semantics. Most efforts focus on covering the \textbf{abnormal side} by enriching the open-ended anomaly semantics. However, anomalies are intrinsically difficult to exhaustively describe. In this work, we enhance the semantics in the \textbf{normal side}. The normal side is more constrained by scene layout, object configuration, and video-specific appearance, and is often more internally consistent within a single surveillance video. Since the final anomaly score is determined by the relative competition between abnormal and normal prompts, the normal side is not merely a background reference; it directly shapes the decision boundary. Nevertheless, it is often treated as generic text or as an auxiliary counterpart to anomaly prompts. 
A few recent methods, such as Cerberus~\cite{zheng2025cerberus}, attempt to model normality more explicitly. However, they still rely on external unlabeled video corpora to learn normality priors and remain ambiguous near the abnormal--normal decision boundary. In contrast, NOVA explicitly models the normal side from the input test video alone, requiring no external data while remaining fully zero-shot.

We identify two structural normal-side limitations of current training-free ZS-VAD frameworks. 
The first one is the \textbf{blurry decision boundary} in LLM-generated normal descriptions.
% First, normal descriptions generated by LLMs are often insufficiently constrained at the linguistic-content level. 
Although existing methods separate normal and abnormal prompts using distinct templates or embedding-level repulsion, semantically ambiguous verbs may still be assigned to the normal prompt set, leading to blurred semantics between normal and abnormal prompts.
For example, words such as ``running'' or ``chasing'' may describe normal activities in some contexts, yet they are visually and semantically close to violent or suspicious events. Once included in normal prompts, these ambiguous terms reduce the separation between normal and abnormal embeddings, inducing systematic scoring errors.

The second limitation is the inherent \textbf{modality gap} between textual and visual embeddings, which persists even with well-designed normal prompts~\cite{liang2022mindgap,song2025reducing}.
A textual normal anchor does not necessarily lie closer to normal video frames than an abnormal textual description does. A fixed text prompt bank sharing across all videos cannot adapt to the scene layout, illumination, camera viewpoint, or background statistics of a specific test video. 
This mismatch reflects a geometric discrepancy between textual and visual embeddings rather than prompt wording, and thus cannot be fully resolved by prompt engineering alone.


To address these limitations, we propose \textbf{NOVA} (\textbf{NO}rmal-side Modeling for ZS-\textbf{VA}D), a training-free framework that explicitly strengthens the normal side at both the linguistic and visual levels. On the language side, NOVA introduces \textbf{Normality-Aware Prompt Construction (NA)}. Instead of only enriching anomaly descriptions, we constrain normal descriptions to avoid anomaly-adjacent ambiguous verbs, bias them toward static and low-motion scenes, and include shared calm anchors for stable normal references. These constraints make the normal prompt set more semantically separable from abnormal prompts, sharpening the \textbf{prompt-contrastive scoring boundary}.

On the visual side, NOVA introduces the \textbf{Visual Normality Anchor (VNA)}, a per-video normal reference constructed directly in the visual embedding space. This anchor exploits the temporal prior in the early frames of the test videos, which are more likely to be normal, and estimates a robust visual normal prototype from these frames. This design bypasses the text-vision modality gap of textual normal anchors and adapts the normal reference to \textbf{each individual video}, while requiring no training samples. 

On top of these two normality-side mechanisms, NOVA adds a lightweight temporal supplement called \textbf{Motion-Aware Stabilization (MAS)}. It combines \textbf{windowed embeddings} and \textbf{motion gating} to reduce frame-level noise and suppress residual false positives in low-motion segments.
The resulting framework remains fully training-free. It uses a frozen vision-language encoder, an offline prompt bank, and test-time visual anchors, without introducing any target-data calibration.


Our contributions are fourfold. First, on the language side, we introduce \textbf{normal-side disambiguation}, a prompt-construction principle that separates normal semantics from the anomaly semantics they compete against, realized as \textbf{Normality-Aware Prompt Construction (NA)}. Second, on the visual side, we introduce \textbf{VNA}, a per-video visual normality reference estimated from the test video itself, with the lightweight temporal supplement MAS layered on top. Third, we recast training-free ZS-VAD as a \textbf{normality-centric problem} and, through controlled ablations and embedding-geometry analysis, show that strengthening the normal side rather than further enriching anomaly semantics is the primary driver of accuracy. Fourth, using only a frozen encoder and test-time anchors, NOVA reaches state-of-the-art accuracy among comparable training-free ZS-VAD methods, achieving 84.82\% AP and 95.07\% AUC on XD-Violence, and 89.86\% AUC on UCF-Crime.


==> backup/sec/2_related.tex <==
% !TEX root = ../main.tex
\section{Related Work}
\label{sec:related}


\subsection{Video Anomaly Detection}
\label{sec:vad}

VAD aims to localize rare abnormal events in long, untrimmed videos. Fully supervised methods rely on frame-level annotations, which incurs substantial annotation cost~\cite{ramachandra2020survey}. Weakly supervised methods reduce this burden by training with video-level labels~\cite{sultani2018real,tian2021weakly,cliptsa2022,wu2024vadclip}. In contrast, unsupervised methods learn anomaly-discriminative cues from unlabeled videos, often exploiting structural assumptions such as the relative rarity~\cite{zaheer2022generative}. These training-based settings have driven much of the progress in VAD, but they typically require task-specific data and learn detection criteria under fixed, dataset-defined notions of normality and abnormality. Recent open-vocabulary and open-world efforts~\cite{li2025anomize,liu2026language} relax this assumption by considering novel categories or user-specified anomaly definitions, yet they still require task-specific learning or adaptation. 


\subsection{Zero-Shot Video Anomaly Detection}
\label{sec:zsvad}

Training-free ZS-VAD seeks to detect potentially unseen anomalous events at inference time using frozen LLMs or VLMs without collecting target-domain data~\cite{zanella2024harnessing,lee2025flashback,askhint2025,shao2025eventvad,ahn2026anyanomaly}. Competing normal and abnormal text prompts have been explored in CLIP-based industrial anomaly detection. WinCLIP~\cite{jeong2023winclip} compares image embeddings with hand-crafted normal and abnormal templates for zero-shot defect classification and segmentation. This prompt-competition view was later extended to videos. VadCLIP~\cite{wu2024vadclip} aligns textual event categories with video segments under weak supervision, and~\cite{dong2024clip} replaces class names with LLM-generated normal and abnormal descriptions. Flashback~\cite{lee2025flashback} moves further toward training-free inference by replacing online LLM reasoning with an offline pseudo-scene memory and by balancing normal and abnormal competition with Repulsive Prompting and Scaled Anomaly Penalization (SAP). NOVA follows this prompt-contrastive line, but focuses on the construction and grounding of normality. Within this line, the two methods most closely related to NOVA are Dong et al.~\cite{dong2024clip} and Flashback~\cite{lee2025flashback}, which both contrast visual representations against LLM-generated normal and abnormal descriptions. Dong et al. still train learnable prompts and temporal modules under video-level weak supervision, whereas NOVA is training-free. Flashback is training-free, but its normal reference remains text-derived. NOVA departs from both on the normal side: it constrains normal-prompt generation to exclude anomaly-adjacent actions and grounds normality in a per-video visual anchor estimated from the test video itself.

Other training-free zero-shot methods use VLMs or MLLMs as reasoning engines rather than prompt competitors. LAVAD~\cite{zanella2024harnessing} generates frame-level scene descriptions with a frozen VLM and converts the description stream into anomaly scores using an LLM. Cerberus~\cite{zheng2025cerberus} combines cascaded VLM reasoning, motion-mask prompting, and behavior-rule deviation detection. VADTree~\cite{li2026vadtree} organizes LLM reasoning through a hierarchical granularity-aware tree, while ASK-Hint~\cite{askhint2025}, EventVAD~\cite{shao2025eventvad}, and PANDA~\cite{Yang2025PANDATG} further explore fine-grained prompting and MLLM-based inference for VAD. LAVIDA~\cite{lavida2026} also uses a multimodal LLM, but relies on external segmentation data to synthesize pseudo-anomalies and is therefore not strictly training-free. These methods improve semantic reasoning but often introduce more complex inference pipelines or additional data assumptions. 

% NOVA instead retains a lightweight prompt-contrastive scorer and improves the normal side used in that competition.

% \noindent\textbf{Differences from text-based ZS-VAD methods.}

\subsection{Normality Modeling}
\label{sec:normalmodeling}

Normality also plays a key role in anomaly detection. One-class VAD methods learn a model of normality from normal-only videos and treat any deviation from it as anomalous~\cite{wang2019gods}.
In weakly supervised VAD, normal videos and snippets also help regularize anomaly scoring~\cite{sultani2018real,tian2021weakly}. However, these approaches obtain normality from training data. In training-free ZS-VAD, the normal side is often represented by text prompts or scene-specific rules constructed before inference~\cite{lee2025flashback}.Cerberus~\cite{zheng2025cerberus} instead models scene-specific normal behavioral rules, but induces them offline from a corpus of sample normal videos. This creates a challenge: the normal representation must be specific enough to compete with anomaly prompts, but must not contain actions that are visually or semantically close to the target anomaly. NOVA addresses this challenge by applying normality-aware prompt construction (NA, Sec.~\ref{sec:prompts}) on the language side and by building a normal anchor on the visual side, without any external normal-video corpus. The latter is related to INP-Former~\cite{luo2025exploring}, which extracts intrinsic normal prototypes directly from a test image. Our VNA extends this observation to the temporal domain by exploiting the prior contained in the early frames of a test video to estimate visual normality.


\subsection{Prompt Design and Modality Gap}
\label{sec:promptdesign}

Prompt design is a key factor in transferring VLMs to downstream tasks. General prompt learning and prompt generation methods show that the construction of textual context can substantially affect recognition behavior: CoOp~\cite{zhou2022coop} learns task-adaptive context vectors from labeled data, whereas CuPL~\cite{pratt2023cupl} uses LLM-generated textual descriptions to improve zero-shot classification. In anomaly detection, prompt design is particularly sensitive because scoring depends on the normality--abnormality contrast rather than a single class name. Image anomaly detection methods such as WinCLIP~\cite{jeong2023winclip} and AnomalyCLIP~\cite{zhou2024anomalyclip} explicitly construct text prompts for normal and abnormal states, while VAD methods extend related textual representations of normality and abnormality to temporally evolving video scenes~\cite{dong2024clip,lee2025flashback}.

Textual prompt engineering alone, however, does not necessarily eliminate the modality gap between text and vision. Prior work shows that contrastive VLMs can embed visual and textual representations in separated regions of a shared feature space, even though the two modalities are trained for cross-modal alignment~\cite{liang2022mindgap,song2025reducing}. For VAD, this implies that textual normality embeddings may not be geometrically close to visual ones. A normal prompt bank may be semantically reasonable, but still provides a weak visual reference. NOVA complements textual prompts by constructing normality directly in the visual embedding space.



==> backup/sec/3_method.tex <==
% !TEX root = ../main.tex
\section{Method}
\label{sec:method}


\subsection{Problem Formulation}
\label{sec:problem_formulation}

Let $V=\{f_t\}_{t=1}^{T}$ be a test video containing $T$ frames, where $f_t\in\mathcal{I}$ denotes the $t$-th image frame. The goal of VAD is to produce a sequence of frame-level anomaly scores $\{s_t\}_{t=1}^{T}$, where $s_t\in[0,1]$, and a higher score indicates a greater likelihood of anomaly. 
Existing methods typically require some form of data dependence to determine the decision boundary, such as frame/video-level annotations, a collection of normal samples, or unlabeled videos for estimating the normal distribution. 
Such dependencies limit practical deployment, as anomalous events are rare and diverse, while privacy concerns and scene changes often require reannotation.


We therefore consider a training-free ZS-VAD setting that removes these dependencies. Given a test video $V$, a footage descriptor $d$ of $V$, and a benchmark-defined anomaly vocabulary $\mathcal{C}$, the model has to estimate the anomaly scores without any training, fine-tuning, hyperparameter selection, or calibration on the target dataset. Frame-level labels $y_t\in\{0,1\}$ remain unavailable throughout.
(For example, $d$ can be as simple as ``surveillance video'' and $\mathcal{C}$ can be \{``fighting'', ``shooting''\}.)



\subsection{NOVA Framework Overview}

NOVA consists of four complementary modules (Fig.~\ref{fig:framework}). 
\textbf{Normality-Aware Prompt Construction (NA)} first builds anomaly descriptions and disambiguated normal descriptions for each anomaly category $c\in\mathcal{C}$ (Sec.~\ref{sec:prompts}).
\textbf{Prompt-contrastive Anomaly Scoring} then uses a frozen vision-language encoder to map frames and prompts from both sides into a shared embedding space, producing category-conditioned scores through anomaly/normal competition (Sec.~\ref{sec:scoring}). On top of this backbone, VNA incorporates early visual normal anchors from the test video itself into the normal-side pool, alleviating the modality gap of textual normal prompts (Sec.~\ref{sec:vna}); MAS further introduces lightweight temporal enhancement at both the embedding and score levels (Sec.~\ref{sec:MAS}). The entire framework trains no parameters.

\begin{figure*}[ht]
\centering
\includegraphics[width=\textwidth]{./pic/framework.png}
\caption{Overview of the NOVA framework. NOVA uses only a frozen vision-language encoder and a pre-constructed prompt bank. It consists of four key stages: normality-aware prompt construction (NA), an anomaly/normal competitive scoring backbone, per-video visual normal anchors (VNA), and MAS with windowed embeddings and motion gating.}
\label{fig:framework}
\end{figure*}


%Normality-Aware 
\subsection{Normality-Aware Prompt Construction}
\label{sec:prompts}

In VAD, the anomaly score is highly sensitive to the relative competition between anomaly and normal prompts. Therefore, normal descriptions are not merely background text; they directly define one side of the decision boundary. This work retains the general paradigm of LLM-generated prompts, but shifts the design focus toward the semantic separability of the normal side. 
All prompt banks are constructed using an LLM, but no LLM is invoked during inference.


For each anomaly category $c\in\mathcal{C}$, our goal is to construct a category-conditioned prompt bank
\begin{equation}
\mathcal{B}_c=\left\{
\mathcal{P}_c =\{p_i^c\}_{i=1}^{M},
\mathcal{N}_c=\{n_j^c\}_{j=1}^{M}
\right\},
\end{equation}
where $\mathcal{P}_c$ contains anomaly-side descriptions, $\mathcal{N}_c$ contains normal-side descriptions, and $M$ is their cardinality.
Each anomaly description $p_i^c \in \mathcal{P}_c$ is expected to cover a subject, an object, and an observable atomic event corresponding to $c$.
Each normal description $n_j^c \in \mathcal{N}_c$, in contrast, should provide \textbf{safe, low-motion, and non-threatening counterexamples} within the same context. A key requirement is that the normal side should not merely describe generic normality, but must avoid \textbf{visually similar normal behaviors} related to $c$; otherwise, the normal descriptions may lie close to the anomaly side in the textual embedding space and weaken the subsequent competitive scoring. 

% The construction pipeline below realizes the normal-side constraints that enforce this requirement; we abbreviate this normality-aware prompt construction as \textbf{NA}.


The prompt-bank construction pipeline consists of four steps. The following describes the procedure for a particular category $c$. Step 4 may be iterated multiple times.

\begin{enumerate}
\item 
\textbf{Confusing verb mining.}
Given $c$ and the footage descriptor $d$, an LLM is invoked to mine a set of category-conditioned yet \textbf{confusing} normal actions,
\begin{equation}
\mathcal{V}_c = \mathrm{LLM}_{\mathrm{verb}}(c, d),
\end{equation}
where each element is a short phrase consisting of 1–3 words that describes a semantically normal action visually similar to $c$.  A single query asks the LLM for 5–8 such actions. For example, $\mathcal{V}_{\mathrm{fighting}}$ may include ``sparring'', ``play wrestling'', and ``horseplay''.

\item 
\textbf{Calm-anchor generation.} 
Conditioned only on $d$, an LLM is invoked to generate a fixed set of calm anchors,
\begin{equation}
\mathcal{A} = \mathrm{LLM}_{\mathrm{anchor}}(d) = \{a_1, \dots, a_K\},
\end{equation}
where each $a_k$ is a low-motion, non-threatening baseline scene of the footage domain, such as ``an empty corridor''. As $\mathcal{A}$ does not depend on $c$, it is generated once and shared across all categories, providing a stable normal reference for the empty or static frames that dominate surveillance footage.

\item 
\textbf{Prompt bank generation.} 
Using a single instruction, an LLM is invoked to produce the anomaly set and an initial normal set,
\begin{equation}
(\mathcal{P}_c, \mathcal{N}_c) = \mathrm{LLM}_{\mathrm{gen}}(c, \mathcal{V}_c, \mathcal{A}, d),
\end{equation}
where $|\mathcal{P}_c| = |\mathcal{N}_c| = M$. The anomaly set $\mathcal{P}_c$ is produced once and fixed, whereas the normal set $\mathcal{N}_c$ may be further revised in step 4.
Following typical anomaly-driven work, $\mathcal{P}_c$ directly describes the category $c$ itself 
(e.g., ``Two people exchanging rapid punches to each other's faces in a hallway'' for category ``fighting''). 
Enforcing $M>K$, $\mathcal{N}_c$ consists of $K$ stable empty-scene descriptions generated from the calm-anchor reference $\mathcal{A}$ (e.g., ``A quiet empty hallway under fluorescent lights with closed doors and no people'') and $M-K$ ordinary normal descriptions (e.g., ``Two people talking calmly beside a doorway with relaxed posture''). 
Terms in the confusing set $\mathcal{V}_c$ are explicitly \textbf{excluded} from the normal descriptions. This constraint prevents semantically ambiguous verbs, such as ``sparring'', from appearing in normality descriptions.
Because the anchor set $\mathcal{A}$ provides examples rather than verbatim templates, the anchor-derived descriptions differ across categories instead of repeating one fixed set of sentences.

\item 
\textbf{Geometry-gated refinement.} 
After step 3, some descriptions in the normal set $\mathcal{N}_c$ may still lean toward the anomaly side in the textual embedding space. This step geometrically detects and rewrites such residual cases.
Assuming a pretrained text encoder $\psi(\cdot)$, we first compute the normalized centroid vector of the anomaly bank,
\begin{equation}
\boldsymbol{\mu}_c^{+}=\mathrm{Normalize}\!\left(\frac{1}{M}
\sum_{p_i^c \in \mathcal{P}_c} 
\psi(T^{+}, p_i^c)\right).
\end{equation}
From the centroid, we compute the ambiguity score $g_j^{c}$ of each normal description $n_j^{c} \in \mathcal{N}_c$ via cosine similarity,
\begin{equation}
g_j^{c}=\psi(T^{-}, n_j^{c})^{\top}\boldsymbol{\mu}_c^{+},
\end{equation}
where a higher value indicates that the normal description is closer to the anomaly side.
$T^+$ and $T^-$ are predefined text prefixes for embedding.
The goal of refinement is to rewrite description $n_j^{c}$ to remove potential ambiguity.
Specifically, $n_j^{c}$ is marked as an \textbf{ambiguous normal} if its $g_j^{c}>\theta$, in which case we invoke an LLM for revision:
$\hat{n}_j^{c}=\mathrm{LLM}_{\mathrm{ref}}(n_j^{c}, c)$ and similarly evaluate its ambiguity score
$\hat{g}_j^{c}$.
The revision replaces $n_j^{c}$ with $\hat{n}_j^{c}$ only if the ambiguity is reduced, i.e., $\hat{g}_j^{c}<g_j^{c}$; otherwise the original $n_j^{c}$ is kept.
The above scoring, marking, and rewriting are then repeated over the current $\mathcal{N}_c$, until the ambiguity scores of all its descriptions drop below $\theta$, until a round accepts no revision, or until a predefined number $R$ of rounds is reached. The resulting $\mathcal{N}_c$, together with $\mathcal{P}_c$, forms the prompt bank $\mathcal{B}_c$.
Values of $T^+$, $T^-$, $\theta$, and $R$ are reported in Sec.~\ref{sec:implementation}.
\end{enumerate}


The procedure above is identical across datasets. 
The only dataset-specific information is the vocabulary $\mathcal{C}$ and the footage descriptor $d$.
In the UCF-Crime dataset, $d=$``a surveillance-video context'', whereas in XD-Violence, $d$=``a movie/web-video context''.

% \red{
% \begin{equation}
% n_j^{c,(t+1)}=
% \begin{cases}
% \hat{n}_j^{c,(t)}, & g_j^{c,(t)}>\theta \ \text{and}\ \hat{g}_j^{c,(t)}<g_j^{c,(t)},\\[2pt]
% n_j^{c,(t)}, & \text{otherwise.}
% \end{cases}
% \end{equation}
% }

% \red{prefix templates $\mathcal{T}_A(\cdot)$, $\mathcal{T}_N(\cdot)$ as inference-time scoring (Sec.~\ref{sec:scoring}). 
% }



\subsection{Prompt-Contrastive Anomaly Scoring}
\label{sec:scoring}

Next, we introduce the base scoring backbone. 
Based on the same text encoder $\psi(\cdot)$ and the prompt bank $(\mathcal{P}_c, \mathcal{N}_c)$, we compute two L2-normalized textual embedding pools:
\begin{equation}
\mathbf{e}_{i}^{+,c}=\psi(T^{+}, p_i^c),\qquad
\mathbf{e}_{j}^{-,c}=\psi(T^{-}, n_j^c),
\end{equation}
where
$p_i^c \in \mathcal{P}_c$ and
$n_j^c \in \mathcal{N}_c$.
% Assuming a pretrained visual encoder $\phi(\cdot)$, we also compute an L2-normalized visual embedding for each frame $f_t$,
Assuming a frozen vision-language encoder whose text tower is the $\psi(\cdot)$ above and whose visual tower is $\phi(\cdot)$, so that textual and visual embeddings live in one shared space, we also compute an L2-normalized visual embedding for each frame $f_t$,
\begin{equation}
\mathbf{x}_t=\phi(f_t)
.
\end{equation}
We adopt Repulsive Prompting and SAP-Softmax from Flashback~\cite{lee2025flashback} as the scoring rule. 
% Anomaly and normal descriptions are wrapped with different prefix templates $T^{+}$ and $T^{-}$, such as ``Anomalous scene:'' and ``Normal scene:'', forming two textual embedding pools:
The similarities between $\mathbf{x}_t$ and the anomaly-side and normal-side embeddings are computed respectively as:
\begin{equation}
r_i^{+,c}=\mathbf{x}_t^\top\mathbf{e}_{i}^{+,c},\qquad
r_j^{-,c}=\mathbf{x}_t^\top\mathbf{e}_{j}^{-,c}.
\end{equation}
To reduce the noise of individual prompts, we apply Top-50\% mean aggregation to estimate the similarities of $f_t$ to both sides:
\begin{equation}
\begin{aligned}
u_t^{+,c} &= \mathrm{TopKMean}_{50\%}(\{r_i^{+,c}\}),\\
u_t^{-,c} &= \mathrm{TopKMean}_{50\%}(\{r_j^{-,c}\}).
\end{aligned}
\end{equation}

\textbf{SAP-Softmax.}
The competition between anomaly and normality is inherently asymmetric. 
Anomaly descriptions are lexically vivid and specific, causing them to attract even normal frames in the shared embedding space.  An unscaled comparison may therefore over-report anomalies. 
SAP~\cite{lee2025flashback} counteracts this bias by discounting the anomaly side with a scaling factor $\alpha<1$, and thus requires an anomaly prompt to accumulate stronger visual evidence before it can outscore the normal side. The two aggregated similarities are scaled by a temperature $\tau$ and turned into a score by a binary softmax:
\begin{equation}
\ell_t^{+,c}=\frac{\alpha u_t^{+,c}}{\tau},\qquad
\ell_t^{-,c}=\frac{u_t^{-,c}}{\tau},
\end{equation}
\begin{equation}
s_t^c=\frac{\exp(\ell_t^{+,c})}
{\exp(\ell_t^{+,c})+\exp(\ell_t^{-,c})}.
\end{equation}
We fix $\alpha$ and $\tau$ across datasets without target-specific tuning, and report their values in Sec.~\ref{sec:implementation}.

Finally, the frame-level anomaly score is obtained by taking the maximum over all categories,
\begin{equation}
s_t=\max_{c\in\mathcal{C}}s_t^c 
.
\end{equation}
While the above scoring rule already defines the anomaly score $s_t$ for frame $f_t$, the next Secs.~\ref{sec:vna} and \ref{sec:MAS} present two additional modules that can be independently plugged into the backbone to improve anomaly detection performance without altering the scoring rule.

%\paragraph{Top-$K$ similarity aggregation.}
%The temporal replacement of $\mathbf{x}_t$ under MAS is described in Sec.~\ref{sec:MAS}. 


\subsection{Visual Normality Anchor (VNA)}
\label{sec:vna}

Even when textual normal descriptions are semantically precise, a modality gap may still exist: textual embeddings and visual frame embeddings are not necessarily aligned geometrically, and textual normal anchors may not lie closer to normal frames than anomaly descriptions in the shared embedding space~\cite{liang2022mindgap,song2025reducing}.

VNA therefore constructs an additional normal reference directly in the visual space. It is based on two key ideas: establishing a normal-prefix prior and avoiding anomalous contamination.

\textbf{Normal-prefix prior.}
Surveillance anomalies are typically sparse and temporally localized events, while normal activities dominate most video segments~\cite{sultani2018real}. This observation motivates using the early frames as a lightweight estimate of the video's normal visual state. VNA exploits this prior from the first $N_{\mathrm{warm}}$ frames of the video without using any annotation. 
%This prior serves as a probabilistic yet stable reference for normality.
This prior is probabilistic and may fail on individual videos, which motivates the robust estimation below.

% \paragraph{Robust anchor estimation.}

\textbf{Anomalous Contamination Avoidance.}
The above warm-up normality assumption may not hold for every video.
% \red{[I don't understand this statement.] When the prefix is contaminated by anomalies, the robust anchor estimation described below mitigates, rather than eliminates, this failure mode.}
Directly averaging the warm-up frames is vulnerable to anomalous contamination in the prefix: a single anomalous frame shifts the prototype toward the anomaly side.
VNA counteracts this through text-informed anomaly weighting.

Specifically, for each warm-up frame $f_t, t \le N_{\mathrm{warm}}$,
we apply the scoring rule of Sec.~\ref{sec:scoring} with VNA disabled to derive a preliminary anomaly score $\hat{s}_t$; the anchor does not exist yet at this point, so the normal side consists of the textual embeddings alone.
Guided by the prompt banks, these scores serve as label-free proxies for the likelihood that the warm-up frames are normal.
We then convert these scores into weights using a softmax mechanism:
\begin{equation}
w_t=
\frac{\exp(-\hat{s}_t/\gamma)}
{\sum_{q=1}^{N_{\mathrm{warm}}}\exp(-\hat{s}_q/\gamma)},
\end{equation}
where $\gamma$ is the anchor temperature that controls how strongly the weights concentrate on the lowest-scoring frames.
Through these weights, we establish a visual normality anchor:
\begin{equation}
\mathbf{a}_{\mathrm{VNA}}=
\mathrm{Normalize}\left(
\sum_{t=1}^{N_{\mathrm{warm}}}w_t\mathbf{x}_t
\right).
\end{equation}

When this VNA module is enabled, the resulting $\mathbf{a}_{\mathrm{VNA}}$ serves as an additional normal embedding to improve anomaly scoring in Sec.~\ref{sec:scoring}.
That is, the textual normal pool is extended from 
$\{\mathbf{e}_{j}^{-,c} | {j=1}..{M} \}$ 
to 
$\{\mathbf{e}_{j}^{-,c} | {j=1}..{M} \}
\cup 
\{\mathbf{a}_{\mathrm{VNA}}\}$.
The same $\mathbf{a}_{\mathrm{VNA}}$ is shared across all categories. 
This design allows the visual-modality normal anchor to \textbf{participate in} the textual-modality normal pool and jointly compete against the textual-modality anomaly pool.
Concretely, the anchor \textbf{extends the normality boundary}, reducing the likelihood of false positives when a normal visual frame lies too close to anomaly descriptions.

We use the same $N_{\mathrm{warm}}$ and anchor temperature $\gamma$ for both datasets, without target-specific tuning, and report their values in Sec.~\ref{sec:implementation}.

%change name

%\subsection{\red{Windowed Embedding and Motion Modulation}}

\subsection{Motion-Aware Stabilization (MAS)}
\label{sec:MAS}

Frame-level scoring is susceptible to single-frame noise and lacks an explicit characterization of event continuity. 
This module leverages motion information to stabilize the anomaly scores. It combines two ideas: windowed embedding and motion gate.


\textbf{Windowed Embedding.}
Given the visual embedding sequence 
$\{\mathbf{x}_t\}_{t=1}^{T}$, we employ moving average with a sliding window of width $W$ (boundary cases omitted for simplicity of presentation),
\begin{equation}
\tilde{\mathbf{x}}_t=
\mathrm{Normalize}\left(
\frac{1}{W}
\sum_{k=-(W-1)/2}^{(W-1)/2}\mathbf{x}_{t+k}
\right).
\end{equation}
This windowed averaging stabilizes the frame-level embeddings. We consistently use $W=5$ in all experiments. When this module is enabled, the visual embedding $\mathbf{x}_t$ in Sec.~\ref{sec:scoring} is replaced by $\tilde{\mathbf{x}}_t$ to improve anomaly scoring.


\textbf{Motion Gating.}
Anomalous events are often accompanied by observable motion, whereas low-motion segments are a common source of false positives. We estimate the local motion strength of frame $f_t$ using the cosine distance between its neighboring original frame embeddings,
\begin{equation}
m_t=1-\mathbf{x}_{t-1}^{\top}\mathbf{x}_{t+1}.
\end{equation}
Note that $\mathbf{x}_{t-1}$ and $\mathbf{x}_{t+1}$ are raw frames (without windowed embedding discussed above).

A soft gate derived from the motion strength is then applied to refine the anomaly score of frame $f_t$:
\begin{equation}
\label{eq:gating}
\bar{s}_t=s_t
\cdot\mathrm{sig}\left(\beta(m_t-\tau_m)\right),
\end{equation}
where $\mathrm{sig}(\cdot)$ denotes the logistic sigmoid, $\tau_m$ is the motion threshold, and $\beta$ is the gate slope; the latter two are fixed across datasets without target-specific tuning, and their values are reported in Sec.~\ref{sec:implementation}. Using a soft gate rather than a hard threshold prevents static anomalies from being completely suppressed: low-motion normal segments are \textbf{down-weighted}, while high-motion segments preserve their \textbf{original} scores. 
When this module is enabled, the anomaly score $s_t$ in Sec.~\ref{sec:scoring} is replaced by $\bar{s}_t$ to improve anomaly detection.
The final scores are then smoothed by a Gaussian temporal filter of bandwidth $\sigma$, a standard post-processing step separate from the embedding- and motion-level operations of MAS.

\textit{Remark.} In practice, $V$ may be obtained by temporally sampling a raw video (e.g., 1:16). The anomaly scores of unsampled frames are obtained by linear interpolation between neighboring scored frames, after which the same gating mechanism in Eq.~\ref{eq:gating} is applied.



==> backup/sec/4_experiment.tex <==
% !TEX root = ../main.tex
\section{Experiments}
\label{sec:experiments}

\subsection{Datasets and Metrics}
\label{sec:datasets}

\noindent\textbf{UCF-Crime}~\cite{sultani2018real}: 
It contains 1900 real-world surveillance videos with 290 test videos, spanning 13 anomaly categories: Abuse, Arrest, Arson, Assault, Burglary, Explosion, Fighting, Road Accident, Robbery, Shooting, Shoplifting, Stealing, and Vandalism, with frame-level binary labels.

\noindent\textbf{XD-Violence}~\cite{wu2020not}: 
It is a multi-scene video dataset sourced from YouTube and movies, covering 6 anomaly categories: Abuse, Car Accident, Explosion, Fighting, Riot, and Shooting, with frame-level binary labels and a test set that mixes videos from different source domains.

As NOVA is entirely training-free, both the training and test sets could ideally be used for evaluation. However, to ensure a fair comparison with the baselines, we use only the test sets in our experiments.

Following the evaluation protocol of prior work~\cite{zanella2024harnessing,ye2025vera,lee2025flashback}, we use frame-level AUC-ROC as the standard metric for UCF-Crime, and frame-level average precision (AP) together with frame-level AUC-ROC for XD-Violence.

\subsection{Implementation Details}
\label{sec:implementation}

We use GPT-5.4-mini-2026-03-17~\cite{openai2026gpt} (OpenAI API) to construct prompt banks $\mathcal{B}_c$ in Sec.~\ref{sec:prompts}. Each anomaly category contains $M=20$ anomaly and $M=20$ normal descriptions. Normal-prompt generation uses category-specific confusing actions and $K=4$ shared calm anchors, followed by geometric filtering and at most $R=3$ refinement rounds with threshold $\theta=0.70$. $K$, $M$, $\theta$, and $R$ are all fixed a priori and are not calibrated on the target dataset. 
To ensure that our method is not sensitive to a particular prompt bank, we independently generate five prompt banks for each category and report the average performance.


% to evaluate prompt sensitivity. The resulting banks are serialized as fixed JSON files and require no LLM calls during video inference.

All experiments run on a single NVIDIA GeForce RTX 4080 SUPER. 
For efficiency, $V$ is sampled from each test video at a 1:16 rate, so the linear interpolation procedure described in the remark of Sec.~\ref{sec:MAS} is applied.
Dataset-level AUC and AP are computed over all frames pooled across the test set: the per-frame scores and their binary labels from every test video are concatenated into a single sequence, over which each metric is computed once. We use PE-Core-L14-336~\cite{meta2025pecore} as the frozen backbone with SAP coefficient $\alpha=0.90$, Softmax temperature $\tau=0.03$, and Gaussian smoothing parameter $\sigma=50.0$. We fix $N_\text{warm}=32$ for both datasets; Sec.~\ref{sec:nwarm} shows that performance is insensitive to this choice. The remaining settings are VNA anchor temperature $\gamma=0.3$, MAS window size $W=5$, motion threshold $\tau_m=0.02$, and gate slope $\beta=20$. The same hyperparameters are used across datasets and prompt seeds.



\subsection{Benchmark Results}
\label{sec:comparison}

Table~\ref{tab:sota} compares NOVA with representative weakly supervised, one-class, unsupervised, zero-shot, and training-free zero-shot methods. To ensure that NOVA is not prompt-sensitive, we report the mean performance over five independently generated prompt banks. 
While NOVA is entirely training-free, requiring neither the target-dataset training split nor task-specific parameter updates or calibration, it remains highly competitive with weakly supervised methods.


\begin{table}[t]
  \centering
  \caption{Comparison with representative VAD methods under different training paradigms. 
  % All values are percentages; higher is better. 
  \textbf{Bold} denotes the best result across all methods, and \underline{underline} denotes the best result within the same paradigm. ``---'' indicates a metric not reported by the original work. $^{\dagger}$LAVIDA and $^{\dagger}$LaGoVAD use external segmentation data to synthesize pseudo-anomalies and are therefore not strictly training-free.}
  \label{tab:sota}
  \resizebox{1.0\columnwidth}{!}{%
 \small
 \setlength{\tabcolsep}{4pt}
  
  \begin{tabular}{llccc}
    \toprule
    &     \multirow{2}{*}[-0.5ex]{%
\begin{tabular}{@{}l@{}}
Method
\end{tabular}} & UCF-Crime & \multicolumn{2}{c}{XD-Violence} \\
    \cmidrule(lr){3-3} \cmidrule(lr){4-5}
    &  & AUC (\%)$\uparrow$ & AP (\%)$\uparrow$ & AUC (\%)$\uparrow$ \\
    \midrule
    \multirow{5}{*}{%
\begin{tabular}{@{}l@{}}
{\textit{Weakly}}\\{\textit{supervised}}
\end{tabular}}
&   RareAnom~\cite{thakare2023rareanom} & 83.56 & --- & 79.89 \\
 &   VERA~\cite{ye2025vera}              & 86.55 & --- & \underline{88.26} \\
 &   CLIP-TSA~\cite{cliptsa2022}         & 87.58 & 82.19 & --- \\
 &   VadCLIP~\cite{wu2024vadclip}        & 88.02 & 84.51 & --- \\
 &   Dong~\cite{dong2024clip}            & 88.52 & --- & --- \\
 &   Holmes-VAD~\cite{zhang2024holmes}   & \underline{89.51} & \underline{\textbf{90.67}} & --- \\
    \midrule
    
   {\textit{One class}} 
    & GODS~\cite{wang2019gods}            & 70.46 & --- & --- \\
    \midrule

        \multirow{4}{*}{%
\begin{tabular}{@{}l@{}}
{\textit{Unsupervised}}
\end{tabular}}
   &
    GCL~\cite{zaheer2022generative}     & 71.04 & --- & --- \\
   & FPDM~\cite{yan2023feature}          & 74.70 & --- & --- \\
   & MULDE~\cite{micorek2024mulde}       & 78.50 & --- & --- \\
   & DyAnNet~\cite{thakare2023dyannet}   & \underline{84.50} & --- & --- \\
    \midrule

        \multirow{2}{*}{%
\begin{tabular}{@{}l@{}}
{\textit{Zero shot}}
\end{tabular}}
&    LaGoVAD$^{\dagger}$~\cite{liu2026language} & 81.12 & 74.25 & --- \\
 &   LAVIDA$^{\dagger}$~\cite{lavida2026} & \underline{82.18} & \underline{90.62} & --- \\
    \midrule

    \multirow{8}{*}{%
\begin{tabular}{@{}l@{}}
{\textit{Training-free}}\\{\textit{zero shot}}
\end{tabular}}
 &   LAVAD~\cite{zanella2024harnessing}  & 80.28 & 62.01 & 85.36 \\
&    AnyAnomaly~\cite{ahn2026anyanomaly} & 80.70 & --- & --- \\
 &   EventVAD~\cite{shao2025eventvad}    & 82.03 & 64.04 & 87.51 \\
 &   VADTree~\cite{li2026vadtree}        & 84.74 & 68.85 & 90.55 \\
 &   PANDA~\cite{Yang2025PANDATG}        & 84.89 & 70.16 & --- \\
 &   Flashback~\cite{lee2025flashback}   & 87.29 & 75.13 & 90.54 \\
 &   ASK-Hint~\cite{askhint2025}         & 89.83 & --- & 90.31 \\
 &   \textbf{NOVA (Ours)} & \textbf{\underline{89.86}} & \underline{84.82} & \textbf{\underline{95.07}} \\
    \bottomrule
  \end{tabular}}
\end{table}

Among training-free zero-shot methods, NOVA achieves the best result on all three metrics. On UCF-Crime, it is comparable to ASK-Hint. On XD-Violence, NOVA improves AP over Flashback~\cite{lee2025flashback} by \textbf{9.69 pp} and AUC over VADTree~\cite{li2026vadtree} by \textbf{4.52 pp}. 
Despite requiring no task-specific training, NOVA remains competitive with several weakly supervised methods. These results highlight the critical role of \textbf{normal-side semantic modeling} in NOVA.



\subsection{Ablation Study}
\label{sec:ablation}

Table~\ref{tab:ablation} reports a full-factorial ablation of NA, VNA, and MAS using the unconstrained LLM-generated prompt base. Here, NA denotes the normality-aware prompt design introduced in Sec.~\ref{sec:prompts}.  When NA is disabled, the normal prompts are the unconstrained LLM-generated ones, without the disambiguation design.


% Each configuration is evaluated with five prompt banks and reported as the mean and standard deviation. The text-side decomposition is provided in Sec.~\ref{sec:decomposition}.

All configurations use the same PE-Core-L14-336 backbone~\cite{meta2025pecore}, scoring hyperparameters, and SAP-Softmax rules. This controlled setup isolates the effects of the enabled components. 
\textbf{Baseline} (all modules disabled) uses unconstrained LLM-generated anomaly and normal prompts, following the competitive scoring of~\cite{lee2025flashback} and~\cite{dong2024clip}. \textbf{NA} enables our normal-prompt generation design, 
\textbf{VNA} adds a per-video visual normal anchor
$\mathbf{a}_{\mathrm{VNA}}$, and \textbf{MAS} adds windowed embeddings and motion gating. 

% The final row enables all three components.

\begin{table}[t]
  \centering
  \caption{Full factorial ablation of NA, VNA, and MAS. Means and standard deviations are reported. 
  % \textbf{Bold} denotes the best result in each column.
  }
  \label{tab:ablation}
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{ccc ccc}
    \toprule
    NA & VNA & MAS & UCF AUC (\%) & XD AUC (\%) & XD AP (\%) \\
    \midrule
    $\times$ & $\times$ & $\times$ & $85.62 \pm 1.41$ & $93.51 \pm 0.48$ & $80.36 \pm 1.51$ \\
    \checkmark & $\times$ & $\times$ & $88.79 \pm 0.50$ & $94.29 \pm 0.45$ & $84.33 \pm 1.60$ \\
    $\times$ & \checkmark & $\times$ & $86.99 \pm 1.03$ & $94.08 \pm 0.41$ & $80.47 \pm 1.45$ \\
    $\times$ & $\times$ & \checkmark & $86.73 \pm 1.27$ & $91.54 \pm 0.23$ & $72.88 \pm 0.64$ \\
    \checkmark & \checkmark & $\times$ & $89.54 \pm 0.45$ & $94.85 \pm 0.30$ & $84.65 \pm 1.35$ \\
    \checkmark & $\times$ & \checkmark & $89.34 \pm 0.61$ & $91.07 \pm 0.36$ & $72.96 \pm 0.66$ \\
    $\times$ & \checkmark & \checkmark & $87.54 \pm 1.00$ & $94.65 \pm 0.29$ & $82.40 \pm 0.91$ \\
    \checkmark & \checkmark & \checkmark & $\mathbf{89.86 \pm 0.43}$ & $\mathbf{95.07 \pm 0.33}$ & $\mathbf{84.82 \pm 0.56}$ \\
    \bottomrule
  \end{tabular}}
\end{table}

Compared to the baseline, NA yields the largest single-factor gain, improving UCF AUC by \textbf{3.17 pp} and XD AP by \textbf{3.97 pp} at no inference-time cost, since it requires only offline prompt construction. VNA improves the three metrics on its own by 1.37, 0.57, and 0.11 pp, respectively. MAS is strongly dataset-dependent; it alone raises UCF-Crime by 1.11 pp but lowers XD-Violence AP by 7.48 pp. The same pattern persists once NA is enabled, where VNA continues to help, while MAS without VNA still costs 11.37 pp of XD AP.

The factorial study further exposes two interactions. First, NA and VNA are sub-additive on UCF-Crime. Their joint gain of 3.92 pp falls short of the 4.54 pp obtained by summing their individual gains, which is consistent with both mechanisms acting on the normal side and therefore capturing partially overlapping structure. On XD-Violence the two are close to additive, indicating that the normal side of movie and web footage is described less redundantly. Second, VNA does not merely mitigate the AP degradation of MAS but fully offsets it. With NA enabled, XD AP rises from 72.96 to 84.82, exceeding even the NA-only level of 84.33 obtained before MAS was added.

These interactions clarify the role of MAS. Once VNA is present, its marginal contribution is small, adding 0.32, 0.22, and 0.17 pp respectively to the three metrics. It nevertheless reduces sensitivity to the prompt bank in a consistent manner. The standard deviation of XD AP falls from a range of 1.35 to 1.60 pp across the four MAS-free configurations to a range of 0.56 to 0.91 pp across the four that enable it. MAS therefore acts as a lightweight temporal stabilizer rather than a primary source of accuracy, and is usable only in combination with VNA. With all three components enabled, NOVA attains the best performance in all metrics.



% \subsection{Decomposition of Normal-Side and Anomaly-Side Contributions}

\subsection{Normal and Anomaly Prompt Analysis}
\label{sec:decomposition}

While prompts play an important role in VAD, NOVA focuses on normal-side modeling. Table~\ref{tab:decomp} presents a systematic analysis of different decompositions of normal and anomaly prompts.
A preliminary model uses templates containing only class names, providing weak anomaly descriptions and no normal-side reference.
Replacing the text with LLM-generated anomaly descriptions improves UCF-Crime but does not reliably improve XD-Violence AP, suggesting that enriching anomaly-side modeling alone is insufficient. 
Introducing additional normal descriptions and jointly scoring anomaly and normal prompts with SAP-Softmax, even without NA, further improves performance.
Applying NA further strengthens the normal side by removing semantically ambiguous descriptions that are close to anomalies. These results highlight the importance of normal-side modeling in NOVA.

\begin{table}[t]
  \centering
  \caption{Decomposition of normal-side and anomaly-side contributions on UCF-Crime and XD-Violence.}
  \label{tab:decomp}
  \resizebox{\columnwidth}{!}{%
  \begin{tabular}{lccc}
    \toprule
    Config & UCF AUC (\%) & XD AUC (\%) & XD AP (\%) \\
    \midrule
    Template, anomaly classes only & 66.85 & 90.99 & 77.94 \\
    LLM, anomaly classes only & $72.50 \pm 2.09$ & $91.81 \pm 0.71$ & $76.44 \pm 2.37$ \\
    LLM, normal+anomaly (no NA) & $85.62 \pm 1.41$ & $93.51 \pm 0.48$ & $80.36 \pm 1.51$ \\
    LLM, normal+anomaly (NA) & \textbf{88.79 $\pm$ 0.50} & 
    \textbf{94.29 $\pm$ 0.45} & \textbf{84.33 $\pm$ 1.60} \\
    \bottomrule
  \end{tabular}}
\end{table}



\subsection{Geometric Analysis of NA}
\label{sec:noconst}

Fig.~\ref{fig:tsne} projects the constrained and unconstrained prompt embeddings with t-SNE for visualization. With NA, the normal (green) and anomaly (red) prompts form more clearly separated groups with less overlap, and the centroid cosine similarity between the two sides decreases from 0.904 to 0.844. This geometric change supports the ablation results in Table~\ref{tab:ablation}, suggesting that NA improves SAP-Softmax by increasing the separability of normal descriptions. In contrast, prior work~\cite{dong2024clip} includes normal descriptions with ambiguous verbs such as ``running'' and ``joggers'', which overlap semantically with anomaly-related actions.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{./pic/fig_tsne_constraint.png}
  \caption{t-SNE projection of UCF-Crime prompt embeddings, where the text embeddings are produced by the PE-Core text encoder over the prompt banks of 5 seeds. Applying NA (left) reduces the anomaly--normal centroid cosine similarity from 0.904 to 0.844, pushing the normal embeddings away from the anomaly descriptions. Stars denote the anomaly/normal centroids.
  % and the annotated value is the cosine similarity between the two centroids, where lower indicates better separation.
  }
  \label{fig:tsne}
\end{figure}



\subsection{Geometric Analysis of VNA and Textual Normal Anchors}
\label{sec:geometric}

Fig.~\ref{fig:pca} projects each video's frame embeddings, category prompt embeddings, $\mathbf{a}_{\mathrm{VNA}}$, and the visual normal centroid $c_n$ onto a per-video PCA plane, where $c_n$ is obtained by normalizing all ground-truth normal-frame vectors to unit size, taking their average, and normalizing the result to unit size again.
$c_n$ is used only as a post-hoc reference and is never involved in VNA construction or inference.
We aggregate statistics over the 140 anomalous UCF-Crime test videos and average each video across five prompt banks. 
We observe three patterns:

\begin{enumerate}
\item 
\textbf{$\mathbf{a}_{\mathrm{VNA}}$ closely matches the visual normal centroid.} The mean cosine similarity between $c_n$ and $\mathbf{a}_{\mathrm{VNA}}$ is 0.969, showing that the score-weighted early-frame prototype closely approximates the full-video normal centroid.
\item 
\textbf{The textual normal anchor aligns poorly with normal frames.} 
The mean cosine similarity between $c_n$ and the textual normal centroid is only 0.167, which is less than one-fifth of the similarity between $\mathbf{a}_{\mathrm{VNA}}$ and $c_n$.
\item 
\textbf{Normal text can be less aligned than anomaly text.} In 94.29\% of the videos, $c_n$ has lower cosine similarity to the textual normal centroid than to the textual anomaly centroid.
\end{enumerate}

These observations support the analysis in Sec.~\ref{sec:promptdesign}: due to the cross-modal gap, the textual normal centroid does not necessarily align reliably with the normal frames, whereas $\mathbf{a}_{\mathrm{VNA}}$ in the visual space provides a reference closer to the video's normal appearance. The distinct clusters of text prompts and visual frames in Fig.~\ref{fig:pca} are also consistent with the CLIP modality gap observed in~\cite{liang2022mindgap,song2025reducing}.

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{./pic/fig_pca_vna.png}
  \caption{Per-video PCA projection of six representative videos. The yellow star denotes the score-weighted $\mathbf{a}_{\mathrm{VNA}}$, and the teal cross denotes the ground-truth normal-frame centroid $c_n$. Blue/red dots are normal/anomalous frames; blue/red triangles are category-specific normal/anomaly prompts; gray markers are prompts from the other categories. 
  % Annotated cosine similarities are computed in the original embedding space.
  }
  \label{fig:pca}
\end{figure}



\subsection{Sensitivity Analysis of \texorpdfstring{$N_\text{warm}$}{Nwarm}}
\label{sec:nwarm}

Table~\ref{tab:nwarm} reports the sensitivity of NOVA to the warm-up window size $N_\text{warm}$. Over an eightfold range from 8 to 64, all three metrics vary within a narrow band: UCF AUC by 0.39 pp, XD AUC by 0.57 pp, and XD AP by 1.67 pp. Sensitivity to this parameter is therefore low, and we fix $N_\text{warm}=32$ for both datasets throughout the experiments without dataset-specific tuning.


\begin{table}[t]
  \centering
  \caption{Sensitivity analysis of $N_\text{warm}$. Results are the mean and standard deviation over five prompt banks. $^{\dagger}$ denotes the default used in the main experiments.}
  \label{tab:nwarm}
  \begin{tabular}{cccc}
    \toprule
    $N_\text{warm}$ & UCF AUC & XD AUC & XD AP \\
    \midrule
    8  & $89.76 \pm 0.40$ & $94.62 \pm 0.38$ & $83.53 \pm 0.68$ \\
    16 & $89.88 \pm 0.41$ & $94.91 \pm 0.35$ & $84.28 \pm 0.59$ \\
    24 & $89.87 \pm 0.42$ & $95.01 \pm 0.33$ & $84.60 \pm 0.58$ \\
    $32^{\dagger}$ & $89.86 \pm 0.43$ & $95.07 \pm 0.33$ & $84.82 \pm 0.56$ \\
    48 & $89.72 \pm 0.45$ & $95.11 \pm 0.33$ & $84.98 \pm 0.54$ \\
    64 & $89.49 \pm 0.47$ & $95.19 \pm 0.33$ & $85.20 \pm 0.53$ \\
    \bottomrule
  \end{tabular}
\end{table}

\subsection{Qualitative Analysis}
\label{sec:qualitative}

Fig.~\ref{fig:perframe} shows the per-frame anomaly scores of three representative UCF-Crime videos under different configurations. With only NA enabled, the anomaly segment forms a clear peak, but the normal segments still contain several relatively high points; after adding VNA, these normal-segment peaks are lowered relative to the main anomaly peak. Adding MAS further smooths some short-lived fluctuations. 
% \red{[don't understand???] Because MAS uses a centered window that includes future frames, the earlier rise in the curve reflects only offline bidirectional temporal aggregation.}刪除


\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{./pic/fig_per_frame_Explosion029_x264.png}
  \includegraphics[width=\linewidth]{./pic/fig_per_frame_Explosion013_x264.png}
  \includegraphics[width=\linewidth]{./pic/fig_per_frame_RoadAccidents016_x264.png}
  \caption{Per-frame qualitative analysis on UCF-Crime. Pink regions denote the annotated ground-truth anomaly frames.
  }
  \label{fig:perframe}
\end{figure}


==> backup/sec/5_conclusion.tex <==
\section{Conclusions}
\label{sec:conclusion}

We presented NOVA, a training-free ZS-VAD framework built on a simple premise: in prompt-contrastive scoring, normal-side modeling deserves as much attention as anomaly-side
NOVA strengthens it at two levels: \textbf{Normality-Aware Prompt Construction (NA)} separates normal textual descriptions from the anomaly-adjacent actions that they would otherwise be confused with, and the \textbf{Visual Normality Anchor (VNA)} grounds normality in the visual embedding space of each test video, bypassing the text--vision modality gap. A lightweight \textbf{Motion-Aware Stabilization (MAS)} module adds temporal robustness on top. Without any training, fine-tuning, or target-data calibration, NOVA reaches 89.86\% AUC on UCF-Crime, surpassing weakly-supervised detectors such as Holmes-VAD, and 95.07\% AUC / 84.82\% AP on XD-Violence, improving AP over the best training-free method by 9.69 pp. 
Controlled ablations and embedding-geometry analyses suggest that normal-side language constraints contribute substantially to performance, and that the visual anchor tends to align more closely with true normality than textual anchors do.

These results also clarify the scope and limitations of NOVA. First, VNA models appearance-level normality rather than temporal dynamics. Second, its early-frame prior may be unreliable when a video begins with anomalous content. Moreover, NOVA estimates a visual normal anchor from a warm-up prefix and applies it to the entire video, making the current framework not fully real-time. These limitations point to several promising directions for future work, including online VNA updating and scene-adaptive normality modeling.

==> backup/sec/temp_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> backup/sec/temp_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
The columns should be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered, and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

The captions of the figures and tables should be in 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centered.  Table captions should be above tables, while figure captions should be below figures.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period, and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use the footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example, at the beginning of the sentence, you can use
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, include the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When citing multiple papers at once, make sure that you cite them in numerical order such as this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \caption{Results.   Ours is better.}
  \label{tab:example}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead, use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise and, therefore, must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence, avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> backup/sec/temp_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets the figure captions and references in a smaller font.
The reason why such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The review process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in 11 pages.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler that should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use the options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Use fractional references (\eg, this line is $087.5$), although in most cases the approximate location would be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please, number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for the reader to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean that some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not mean that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of our previous paper [1], and show that it is inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of the paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time that covers similar or overlapping material, you may need to refer to that submission to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, do not assume that the reviewers will read this material.

Sometimes your paper is about a problem that you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think that it is likely that the new article was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
However, for your results, you should not identify yourself and should not mention your participation in the challenge.
Instead, present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison with other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has only two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/temp_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/temp_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
The columns should be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered, and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

The captions of the figures and tables should be in 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centered.  Table captions should be above tables, while figure captions should be below figures.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period, and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use the footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example, at the beginning of the sentence, you can use
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, include the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When citing multiple papers at once, make sure that you cite them in numerical order such as this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \caption{Results.   Ours is better.}
  \label{tab:example}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead, use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise and, therefore, must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it is almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence, avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/temp_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets the figure captions and references in a smaller font.
The reason why such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The review process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in 11 pages.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler that should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use the options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Use fractional references (\eg, this line is $087.5$), although in most cases the approximate location would be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please, number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for the reader to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean that some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not mean that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of our previous paper [1], and show that it is inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper, we present a performance analysis of the paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time that covers similar or overlapping material, you may need to refer to that submission to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, do not assume that the reviewers will read this material.

Sometimes your paper is about a problem that you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think that it is likely that the new article was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
However, for your results, you should not identify yourself and should not mention your participation in the challenge.
Instead, present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison with other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has only two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}

